Cyber-Physical Specification Mismatches

Embedded systems use increasingly complex software and are evolving into cyber-physical systems (CPS) with sophisticated interaction and coupling between physical and computational processes. Many CPS operate in safety-critical environments and have stringent certification, reliability, and correctness requirements. These systems undergo changes throughout their lifetimes, where either the software or physical hardware is updated in subsequent design iterations. One source of failure in safety-critical CPS is when there are unstated assumptions in either the physical or cyber parts of the system, and new components do not match those assumptions. In this work, we present an automated method towards identifying unstated assumptions in CPS. Dynamic specifications in the form of candidate invariants of both the software and physical components are identified using dynamic analysis (executing and/or simulating the system implementation or model thereof). A prototype tool called Hynger (for HYbrid iNvariant GEneratoR) was developed that instruments Simulink/Stateflow (SLSF) model diagrams to generate traces in the input format compatible with the Daikon invariant inference tool, which has been extensively applied to software systems. Hynger, in conjunction with Daikon, is able to detect candidate invariants of several CPS case studies. We use the running example of a DC-to-DC power converter, and demonstrate that Hynger can detect a specification mismatch where a tolerance assumed by the software is violated due to a plant change. Another case study of an automotive control system is also introduced to illustrate the power of Hynger and Daikon in automatically identifying cyber-physical specification mismatches.

==> case_study.tex <==
\subsection{Buck Converter with Hysteresis Control}
\seclabel{case_study}
%
Next, we describe a CPS case study used throughout the remainder of the \papertype for illustrating concepts.
%
The case study is a DC-to-DC power converter (like buck, boost, and buck-boost converters)~\cite{nguyen2014arch}, all of which have similar modeling, but we focus particularly on a buck converter.
%
A buck converter takes an input voltage of say $5$V and ``bucks'' or drops the voltage to some lower DC voltage, say $2.5$V.
%
These circuits are used in many electronic devices (e.g., personal computers, cellphones, embedded systems, aircraft, satellites, cars).
%
These circuits are also used as modular components in a variety of novel power electronics architectures, such as AC/DC microgrids and distributed DC-to-AC multilevel inverters~\cite{nguyen2014tec}.
%
For these converters, one of the physical specifications is that, at steady-state, the output voltage is always bounded within a tolerance of a desired (reference) voltage (e.g., $\Vout(t)= \Vref(t) \pm \epsilon$).
%
We will formalize specifications and mismatches in~\secref{spec_mis}.
%
As a prelude, we highlight that \toolhynger finds this candidate invariant (that can be shown to be an actual invariant when modeled as a  hybrid automaton~\cite{johnson2012peci,hossain2013peci,nguyen2014arch}).


%
Additionally, experimental results for additional examples using \toolhynger are presented later in~\secref{experiment}.
%
%although we do not have space to describe them in detail in this \papertype.
%
The general architecture of the case study we focus on consists of a plant (physical system) model and a controller (cyber model/software), along with models of actuators and sensors interfacing the plant and controller, that is generally depicted in \figref{feedback_controller}.
%
The sensor model performs quantization and sampling, as would occur in typical analog to digital conversion (ADC) used to digitize analog signal measurements.
%
The actuator models likewise perform the inverse process of digital to analog conversion (DAC) to convert the digital (cyber) signals to analog signals.
%
An overview of the buck converter system architecture appears in the root SLSF diagram of~\figref{case_study_overview}.


%\begin{figure}[t!]%
	%\centering%
	%\includegraphics[width=\columnwidth]{image/case_study_overview.pdf}%
	%\addtikz{image/case_study}{1}%
	%\vspace{-0.5em}%
	%\caption{General CPS case study architecture overview in SLSF.  The system is composed of a plant (physical system) model, a controller (software/cyber), and potentially sensor and actuator models.  The cyber model uses some of the physical model output states to determine a control action or input.  For the buck converter, the plant model is described as a hybrid automaton in~\figref{automaton_buckboost}, the controller appears in~\figref{case_study_controller_hysteresis}, and the sensor model appears in~\figref{case_study_sensor}.}%
	%\caption{General CPS case study architecture overview in SLSF.  The system is composed of a plant (physical system) model, a controller (software/cyber), and potentially sensor and actuator models.  The cyber model uses some of the physical model output states to determine a control action or input.  For the buck converter, the closed-loop model can be represented as a hybrid automaton in~\figref{automaton_buckboost}, the controller in SLSF appears in~\figref{case_study_controller_hysteresis}, and the sensor model appears in~\figref{case_study_sensor}.}%
	%\figlabel{case_study_overview}%
	%\vspace{-0.75em}
%\end{figure}%

%\begin{figure}[t!]%
	%\centering%[width=\columnwidth]
	%\includegraphics[width=\imagewidthBigger\columnwidth]{image/case_study_sensor.pdf}%
	%\vspace{-0.5em}
	%\caption{Stateflow model of sensor with a sample-and-hold for the buck converter case study.}
	%\figlabel{case_study_sensor}%
	%\vspace{-0.5em}
%\end{figure}%

\paragraph*{Buck Converter Plant Model}
%
We briefly describe a switched-system plant model of a buck converter, but in-depth derivations of these models and non-idealized versions in power electronics textbooks~\cite{severns1985book,erickson2004book}.
%
The buck converter plant may be modeled as a hybrid automaton as described in detail~\cite{johnson2012peci,hossain2013peci,nguyen2014arch,nguyen2014tec}.
%
%%See~\figref{buck} for a circuit diagram of the buck converter.
%%
%%
%\begin{figure}[t!]%
	%\centering%
	%\includegraphics[height=1.4cm]{image/buck.pdf}%width=\columnwidth,
	%\vspace{-0.5em}
	%\caption{Buck converter circuit---a DC input $\Vs$ is decreased to a lower DC output $V_o = \Vout$.}%
	%\figlabel{buck}%
	%\vspace{-0.5em}
%\end{figure}%



%\begin{table}[tb]%
	%\scriptsize%
	%\centering%
	%\scriptsize%
	%\begin{tabular}{|l|c|l|}%
		%\hline
		%Component / Parameter Name & Symbol & Value  																		\\
		%\hline
		%Source Input Voltage										& $\Vs$							&	$24$ V				\\
		%Desired Output (Reference) Voltage					& $\Vref$					  &	$12$ V				\\
		%Actual Output Voltage					  & $\Vc = \Vout$			&	$12$ V	$\pm \ \Vripple$			\\
		%Hysteresis Band Tolerance				& $\Vtol$					  &	$0.2$ V				\\
		%Voltage Ripple Tolerance				& $\Vripple$				&	$0.6$ V				\\
		%Load Resistance									& $R$								&	$10 \Omega$			\\
		%Capacitor												& $C$								&	$2.2$ mF				\\
		%Inductor												& $L$								&	$2.65$ uH					\\
		%\hline 
	%\end{tabular}%
	%\vspace{0.1cm}%
	%\caption{Example buck converter parameter values and variations.}%
	%\tablabel{buck_parameter}%
%\end{table}%
%






The buck converter has two real-valued state variables modeling the inductor current $i_L$ and the capacitor voltage $V_C$.
%
%depicted in~\figref{buck}.
%
These state variables are written in vector form as: $x = \left[ i_L; V_C \right]$.
%
%Standard realizations of these converters utilize PWM to switch between the connected and disconnected modes, so an additional real-valued state variable $\tau$ models real-time ($\dot{\tau} = 1$).
%
The dynamics of the continuous variables in each mode $m \in \{\mathit{Open}, \mathit{Close}\}$---in short, $o$ and $c$---are specified as linear (affine) differential equations: $\dot{x} = A_m x + B_m u$, where $u = \Vs$.
%
\figref{automaton_buckboost} shows a hybrid automaton model for the converter, where the plant is easily translated to a continuous-time Stateflow model (see, e.g.,~\cite{nguyen2014arch}), and the controller is translated to discrete-update Stateflow model. In~\figref{automaton_buckboost}, $\LabelActionBuck$ is a synchronization label and $mode$ is a discrete control signal.
%
A closed-loop controller for this buck converter is a hysteresis controller, which changes the mode of the buck converter plant based on the measured output voltage~\cite{hossain2013peci}.
%
The $A_m$ matrices consist of $L > 0$, $R > 0$, $C > 0$ real-valued constants, respectively representing inductance (in Henries), resistance (in Ohms), and capacitance (in Farads).
%
%See~\tabref{dynamics} for the $A_m$ matrices and $B_m$ vectors that specify the dynamics for the converter.
%


\def\BuckStateVector{\left[ \begin{array}{c} \iL \\ \Vc \end{array} \right]}
\def\BuckStateVectorDot{\left[ \begin{array}{c} \iLdot \\ \Vcdot \end{array} \right]}

%\begin{figure}[t!]%
	%\centering%
	%\normalsize
	%\begin{adjustbox}{max size={\columnwidth}{0.75\textheight}}%
	%\begin{tikzpicture}[>=stealth',shorten >=1pt,auto,node distance=8cm,font=\normalsize]
		%\tikzstyle{every state}=[font=\normalsize,rectangle,rounded corners]
		%\tikzstyle{every state}=[minimum size=6cm,font=\normalsize]
	%	\node	[initial,state]		(open) 	{\makecell[c]{$\text{Open}$\\$\BuckStateVectorDot = \left[ \begin{array}{cc} 0 & -\frac{1}{L} \\ \frac{1}{C%} & -\frac{1}{R C} \end{array} \right] \BuckStateVector$}};
		%\node[state] (closed)      	[right of=open]		{\makecell[c]{$\text{Close}$\\$\BuckStateVectorDot = \left[ \begin{array}{cc} 0 & -\frac{1}{L%} \\ \frac{1}{C} & -\frac{1}{R C} \end{array} \right] \BuckStateVector + \left[ \begin{matrix} \frac{1}{L}\\ 0 \end{matrix} \right] \Vs$}};
		%\node	[state]		(dcm) [right of=closed]	{\makecell[c]{$\text{DCM}$\\$\BuckStateVectorDot = \left[ \begin{array}{cc} 0 & 0 \\ 0 & -\frac{1}{R C} \end{array} \right] \BuckStateVector$\\$\iL \leq 0$}}; 
		%\path[->]			(closed)	edge[bend left] node{\makecell[c]{$mode==2$}} (open); 
		%\path[->]			(open)	edge[bend left] node{\makecell[c]{$mode==1$}} (closed); 
		%\path[->]			(open)	edge[bend right] node[below]{\makecell[c]{$\iL \leq 0$}} (dcm); 
		%\path[->]			(dcm)	edge[bend right] node[above]{\makecell[c]{$\Vc - \Vref \geq \Vtol$}} (closed);
	%\end{tikzpicture}%
	%\end{adjustbox}%
	%\vspace{-1em}%
	%\caption{Hybrid automaton model of the buck converter plant. A corresponding continuous-time Stateflow model is used for the plant.}%
	%\figlabel{automaton_buckboost}%
	%\vspace{-1em}%
%\end{figure}%

\begin{figure}[t!]%
	\centering%
	%\scriptsize{
	%\begin{adjustbox}{max size={0.99\columnwidth}{0.66\textheight}}%
	\scalebox{0.75}{
	\begin{tikzpicture}[>=stealth',shorten >=1pt,auto,node distance=9cm,font=\normalsize]
		\tikzstyle{every state}=[font=\normalsize,rectangle,rounded corners]
		%
		\node	[state]		(open) 	{\makecell[c]{$\text{Open}$\\$\BuckStateVectorDot = \left[ \begin{array}{cc} 0 & -\frac{1}{L} \\ \frac{1}{C} & -\frac{1}{R C} \end{array} \right] \BuckStateVector$\\$mode = 1 \wedge \iL \geq 0 \wedge \Vc \leq \Vref + \Vtol$}};
		%
		\node[state] (closed)      	[right=2mm of open]		{\makecell[c]{$\text{Closed}$\\$\BuckStateVectorDot = \left[ \begin{array}{cc} 0 & -\frac{1}{L} \\ \frac{1}{C} & -\frac{1}{R C} \end{array} \right] \BuckStateVector + \left[ \begin{matrix} \frac{1}{L}\\ 0 \end{matrix} \right] \Vs$\\$mode = 2 \wedge \iL \geq 0 \wedge \Vc \geq \Vref - \Vtol$}};
		%
		\node	[state]		(dcm) [right=2mm of closed]	{\makecell[c]{$\text{DCM}$\\$\BuckStateVectorDot = \left[ \begin{array}{cc} 0 & 0 \\ 0 & -\frac{1}{R C} \end{array} \right] \BuckStateVector$\\$mode = 1 \wedge \iL \leq 0$}}; 
		%
		\path[->]			(closed)	edge[bend left] node[below] {\makecell[c]{$\LabelActionBuck$}} (open); 
		%
		\path[->]			(open)	edge[bend left] node[above] {\makecell[c]{$\LabelActionBuck$}} (closed);
		%
		\node[coordinate] (c1) [above=10mm of open.north] {};
		\node[coordinate] (c2) [above=10mm of dcm.north] {};
		\draw[->]			(open.north) -- (c1) -- (c2) to node[right] {\makecell[c]{$\LabelActionBuck$\\$\iL \leq 0$}} (dcm); 
		%
		\path[->]			(dcm)	edge[bend right] node[above]{\makecell[c]{$\LabelActionBuck$}} (closed);
		%
		\node (init) [above=3mm of closed,xshift=-15mm] {start};
		\draw[->] (init) -- (open.north -| init);
		\node (plant) [above=10mm of open,xshift=-25mm] {Plant};
		\node [coordinate] (p1) [above=3mm of plant,xshift=-7mm]{};
		\node [coordinate] (p2) [above=3mm of plant,xshift=166mm]{};
		\node [coordinate] (p3) [below=48mm of p2]{};
		\node [coordinate] (p4) [below=48mm of p1]{};
		\node [coordinate] (pmid23) [below=24mm of p2]{};
		\node [coordinate] (pmid23r) [right=5mm of pmid23]{};
		\node [coordinate] (pmid14) [below=24mm of p1]{};
		\node [coordinate] (pmid14l) [left=5mm of pmid14]{};
		\draw [dashed] (p1)-- (p2) -- (p3) -- (p4)-- (p1){};

	%
		\node	[state]		(controller_open)[below=34mm of open.south, xshift = 30mm]{\makecell[c]{$\text{Open}$\\$mode = 1 \wedge \Vc \geq \Vref - \Vtol$}};
		\node	[state]		(controller_closed) [right=14mm of controller_open]	{\makecell[c]{$\text{Closed}$\\$mode = 2 \wedge \Vc \leq \Vref + \Vtol$}}; 
		\path[->]			(controller_open)	edge[bend left] node[above] {\makecell[c]{$\LabelActionBuck$\\$\Vc \leq \Vref - \Vtol$\\$mode := 2$}} (controller_closed); 
		\path[->]			(controller_closed)	edge[bend left] node[below] {\makecell[c]{$\LabelActionBuck$\\$\Vc \geq \Vref + \Vtol$\\$mode := 1$}} (controller_open);
		%\node[coordinate] (c1) [below=10mm of open.south, xshift=-15mm] {};
		%\node[coordinate] (c2) [below=10mm of open.south,xshift=-5mm]  {};
		%\draw[->]			(open.south) -- (c1) -- (c2) to node[below] {\makecell[c]{$\Vc < \Vref - \Vtol$}} (open); 
		\path[->]			(controller_open)	edge[loop below, in=225, out=315] node{\makecell[c]{$\LabelActionBuck$\\$\Vc > \Vref - \Vtol$}} (controller_open); 
		%
		\path[->]			(controller_closed)	edge[loop below, out=225, in=315] node{\makecell[c]{$\LabelActionBuck$\\$\Vc < \Vref + \Vtol$}} (controller_closed); 
		%
		\node (init) [above=3mm of controller_closed,xshift= 15mm] {start};
		\draw[->] (init) -- (controller_closed.north -| init);
		\node (controller) [above=10mm of controller_open, xshift=-25mm] {Controller};
		\node [coordinate] (co1) [above=6mm of controller,xshift=-10mm]{};
		\node [coordinate] (co2) [above=6mm of controller,xshift=110mm]{};
		\node [coordinate] (co3) [below=52mm of co2]{};
		\node [coordinate] (co4) [below=52mm of co1]{};
		\node [coordinate] (comid23) [below=26mm of co2]{};
		\node [coordinate] (comid14) [below=26mm of co1]{};
		\node [coordinate] (comid23r) [below=52mm of pmid23r]{};
		\node [coordinate] (comid14l) [below=52mm of pmid14l]{};
		\node (vc_input) [below=30mm of pmid23r,xshift=-5mm]{$\Vc$};
		\node (mode_input) [below=30mm of pmid14l,xshift=5mm]{$mode$};
		\draw [dashed] (co1)-- (co2) -- (co3) -- (co4)-- (co1){};
		\draw [dashed,->] (pmid23)-- (pmid23r) -- (comid23r)--(comid23){};
		\draw [dashed,->] (comid14)-- (comid14l) -- (pmid14l)-- (pmid14){};
				%\vspace{-1em}
	\end{tikzpicture}%
	}
	%\end{adjustbox}%
	%\vspace{-1em}%
	\caption{A hybrid automaton models the buck converter plant with hysteresis controller. %A corresponding continuous-time Stateflow model with continuous update is used for the plant, and a discrete-update Stateflow model is used for the controller.%\commentluan{I will try to create the hybrid automaton model with the array and averaging stuff. Here, we use this current version to better describle a closed-loop CPIOA.}
	}%
	\figlabel{automaton_buckboost}%
	%\vspace{-1em}%
\end{figure}%
%\todo{double check DCM dynamics}
%\todo{fix layout}



%\begin{figure}[t!]%
	%\centering%
	%\includegraphics[width=\imagewidth\columnwidth]{image/case_study_plant.png}%
	%\vspace{-0.5em}%
	%\caption{Stateflow continuous-time model of the buck converter plant, which is effectively an instantiation of the hybrid automaton of~\figref{automaton_buckboost} in a continuous-time Stateflow diagram.}
	%\figlabel{case_study_plant}%
	%\vspace{-1em}%
%\end{figure}%



\paragraph*{Closed-Loop Buck Converter}
%
Many control strategies exist for closed-loop feedback control of buck converters.
%
The control strategy we will consider is hysteresis control, which operates intuitively similar to typical heating, ventilation, and cooling (HVAC) control with a thermostat.
%
The converter is meant to transform a given source voltage $\Vs$ to create an output voltage $\Vout$ approximately equal to a desired reference voltage (or set-point) $\Vref$.
%
To accomplish this, the switch controlling whether $\Vs$ is connected to the output or not is toggled depending on whether $\Vout > \Vref$ or $\Vout < \Vref$.
%
In practice, to avoid switching too often, a hysteresis band is used and switches occur when $\Vout > \Vref + \Vtol$ or $\Vout < \Vref - \Vtol$.
%
The choice of $\Vtol$, along with the system dynamics, will determine the voltage ripple $\Vripple$ about the set-point $\Vref$.
%
Typical specifications require the voltage ripple to be small, so that the output voltage $\Vout$ is approximately $\Vref$, that is, $\Vripple$ is chosen so that for $\Vout = \Vref \pm \Vripple$, we have $\Vout \approx \Vref$.
%
We note that $\Vtol$ appears in the controller~\figref{case_study_controller_hysteresis}, so an assumption is made about the relationship between $\Vtol$ and $\Vripple$ in software.


%\begin{figure}[t!]%
	%\centering%[width=\columnwidth]
	%\includegraphics[width=\imagewidthBigger\columnwidth]{image/case_study_sensor.pdf}%
	%\vspace{-0.5em}
	%\caption{Stateflow model of sensor with a sample-and-hold for the buck converter case study.}
	%\figlabel{case_study_sensor}%
	%\vspace{-0.5em}
%\end{figure}%

%\begin{figure}[t!]%
	%\centering%
	%\includegraphics[width=\columnwidth]{image/case_study_controller_hysteresis.pdf}%
	%\vspace{-0.5em}%
	%\caption{Stateflow model of buck-converter voltage hysteresis controller.  The digitized output voltage from the buck-converter plant is %used to determine the mode of the switch.  Here, $\Vtol$ is denoted by the variable $\mathtt{Vtol}$, $\Vref$ is $\mathtt{Vref}$. We highlight %that the controller computes a moving average by summing an array.  With \toolhynger and Daikon, we automatically infer that the result of %this is the sum of the samples, similar to the sum return specification shown in~\figref{sum_array_invariants} found for the C function in~%\figref{sum_array}.}
	%\figlabel{case_study_controller_hysteresis}%
	%%\vspace{-1.5em}%
%\end{figure}%



% for afrl report
%\subsection{Electrical Microgrid}
%\seclabel{microgrid}
%%
%Buck-converters are used as subcomponents in many systems, such as electrical microgrids~\cite{nguyen2014tec}.
%%
%An example appears in~\figref{array}, where $N$ inverter modules are used to converter solar power to electrical power.
%%
%%
%\begin{figure}[t!]%
	%\centering%
	%\includegraphics[height=5cm]{image/array.pdf}%width=\columnwidth,
	%\caption{Solar array architecture using a multilevel inverter for DC-to-AC conversion and consisting of $N$ buck converters.}%
	%\figlabel{array}%
%\end{figure}%





